TrustRoboReward: Preference-Ordered Isotonic Score Editing for Multi-Paradigm Robot Reward Models

Reward models are a bottleneck for reinforcement learning in embodied AI. Long-horizon robotic manipulation requires scalable vision feedback beyond handcrafted rewards or task-specific annotations. Existing open-source VLM reward judges like RoboReward adopt simple 1--5 trajectory progress scoring, lacking pairwise preferences for RLHF, DPO and Bradley-Terry frameworks, while failing to optimize video scene understanding. Augmenting RoboReward with pairwise comparison and video-QA supervision causes inconsistency between pairwise preferences and pointwise scores, introducing training noise and hurting downstream performance---an issue aggregation methods such as TrustJudge cannot resolve. To address this, we propose TrustRoboReward, a multi-paradigm reward modeling framework equipped with Preference-Ordered Isotonic Score Editing (POISE). We construct a unified four-paradigm dataset with trajectory progress scoring (Score-A), video-QA answer quality scoring (Score-B), and their pairwise counterparts (Pair-A, Pair-B). Pairwise labels align better with human judgment than pointwise scores, inspiring us to calibrate pointwise scores to avoid score-pair reversals against pairwise preferences. POISE rectifies pointwise scores and eliminates cross-paradigm reversal conflicts unresolved by TrustJudge. Theoretically, POISE reduces score-pair reversal conflicts from 20.15% to 0%, whereas TrustJudge retains 20.46% conflicts on the same corpus. Evaluated on our benchmark, Qwen3-VL-4B trained with POISE achieves an overall reward score of 77.96%, nearly matching GPT-5-mini (78.09%, gap 0.13%) and outperforming the strongest RoboReward-4B baseline by 10.13%. It also lifts test-time score-pair consistency to 71.90%, exceeding RoboReward-4B (57.26%) and GPT-5-mini (68.09%). Integrating TrustJudge aggregation during inference boosts the overall score to 78.57%, surpassing the GPT-5-mini teacher model.

==> backup_data_construction.tex <==
%-------------------------------------------------------------------
\subsection{Data Construction}
\label{sec:exp:data}

\paragraph{Four supervision views.}
Starting from the RoboReward~\citep{roboreward} dataset, we construct
four reward-supervision views, formed by crossing two output formats
(pointwise scoring vs.\ pairwise comparison) with two input modalities
(trajectory progress vs.\ video question answering). The
trajectory-progress modality (denoted \textsc{A}) takes the original
RoboReward instruction as the question and a robot execution video as
the answer; the VQA modality (denoted \textsc{B}) fixes the question
\emph{``What are the objects and actions of the robot arm in the
video?''}, takes the trajectory video as input, and treats the
RoboReward instruction associated with that video as the candidate
textual answer to be judged. Concretely:
\textbf{Score-A} prompts the reward model to assign a $1$--$5$ score
to a single (instruction, video) pair, matching the RoboReward
formulation;
\textbf{Score-B} prompts it to assign a $1$--$5$ score to a single
(video, fixed question, candidate instruction-as-answer) triple;
\textbf{Pair-A} prompts it to choose, among two candidate videos for
the same instruction, the one that better completes the command (or
to declare a tie);
\textbf{Pair-B} prompts it to choose, among two candidate
instructions-as-answers for the same (video, fixed question), the
one that more correctly describes the scene (or to declare a tie).

\paragraph{Subclass-restricted pair sampling.}
Forming pairs over the entire corpus would explode the dataset
quadratically. We therefore exploit the existing subclass partition
in RoboReward and only sample pairs within a subclass, restricted to
videos that belong to the same group inside that subclass. Some
subclasses contain instructions that have only one associated video
and therefore admit no pairwise neighbor; we call these
\emph{isolated} samples. Isolated samples cannot enter Pair-A or
Pair-B and are routed exclusively into the Score-A and Score-B
training sets for SFT, bypassing the downstream DAG and PAVA stages
since they participate in no preference structure.

\paragraph{Train and test pool sizes.}
After pair sampling we obtain $45{,}072$ Score-A, $45{,}072$ Score-B,
$44{,}528$ Pair-A, and $47{,}020$ Pair-B training samples,
totalling $181{,}692$ training samples. The held-out gold evaluation
set contains $2{,}831$ Score-A, $2{,}831$ Score-B, $672$ Pair-A, and
$696$ Pair-B examples, totalling $7{,}030$ samples. On the pairwise
side, Pair-A and Pair-B at training time correspond to $22{,}264$ and
$23{,}510$ unique unordered pairs respectively, each instantiated in
both the forward and the swapped candidate-presentation orderings.

\paragraph{Single-decode teacher distillation.}
We distill all training labels with a single teacher,
\textbf{GPT-5-mini}, using greedy decoding ($\text{temperature}=0$),
one decode per sample, and at most four parse retries to recover a
machine-readable discrete label; samples that still fail parsing are
discarded. For pairwise samples, the teacher is queried under two
candidate-presentation orderings, the \emph{forward} ordering
$(c_1,c_2)$ and the \emph{swapped} ordering $(c_2,c_1)$, with $c_1$
and $c_2$ the two candidates being compared; the two judgments are
then merged into a canonical label
$\ell\in\{\textsc{L},\textsc{R},\textsc{T}\}$, where \textsc{L}
denotes that the first candidate $c_1$ is preferred, \textsc{R} that
the second candidate $c_2$ is preferred, and \textsc{T} that the two
orderings disagree or that the teacher declared a tie. For pointwise
samples the teacher's discrete $1$--$5$ score and chain-of-thought
rationale are stored verbatim. The same single-decode protocol is
used for all training-time corpora throughout the paper, so any
differences between recipes are attributable to the corpus
construction rather than the teacher decoding budget.

\paragraph{Distillation statistics.}
On Score-A the teacher distillation produces a $1/2/3/4/5$ score
distribution of $17{,}039 / 9{,}299 / 5{,}969 / 5{,}518 / 7{,}247$;
on Score-B the corresponding distribution is
$7{,}334 / 4{,}980 / 17{,}591 / 7{,}405 / 7{,}762$. On the pairwise
side, the canonical label distributions
$\textsc{L}/\textsc{R}/\textsc{T}$ are
$20{,}046 / 18{,}726 / 5{,}756$ for Pair-A and
$21{,}528 / 20{,}022 / 5{,}470$ for Pair-B. In Pair-A,
$1{,}974$ unique pairs are \emph{order-inconsistent}: their forward
and swapped judgments cannot be reconciled into a single canonical
label \textsc{L} or \textsc{R}; for Pair-B this number is $2{,}685$.
Cross-comparing the canonical pairwise labels against the
corresponding pointwise scores yields $7{,}498$ \emph{score--pair
conflicts} on Pair-A and $7{,}107$ on Pair-B, where the pairwise
winner is ranked strictly below its opponent on the $1$--$5$ scale.
These two statistics --- cyclic / order-inconsistent pairs and
score--pair conflicts --- are the direct inputs to the DAG and PAVA
stages and motivate the train-data routing of \S\ref{sec:method};
they are not a side product of post-hoc data cleaning but the core
signal on which our split design is based.

\paragraph{Six labeled splits.}
Routing the conflict statistics above through our pipeline
(\S\ref{sec:method}) induces six labeled splits over the distillation
corpus, which serve as the primitive over which all training recipes
are specified.
$\mathcal{S}_1$ and $\mathcal{P}_1$ are the \emph{raw} pointwise and
pairwise distillations.
DAG-based de-cycling of $\mathcal{P}_1$ produces the
\emph{cleaned pairwise} split $\mathcal{P}_2$ ---
preferences whose chain-of-thought is still consistent with the
post-DAG label, and therefore admissible for SFT --- and the
\emph{residual pairwise} split $\mathcal{P}_3$, whose chain-of-thought
no longer matches the revised label and which is reserved for RL,
where rationale supervision is not required. Propagating the cleaned
pairwise structure back to the pointwise side via PAVA induces an
analogous partition of the pointwise corpus into a SFT-admissible
$\mathcal{S}_2$ and an RL-only residual $\mathcal{S}_3$.

\paragraph{Test gold annotation.}
The held-out gold labels for the $7{,}030$-sample evaluation set are
produced by \textbf{Gemini-3.1-Pro-Preview}~\citep{gemini2025} under
the same single-decode protocol used at training time
($\text{temperature}=0$, one decode per sample). Because the training
teacher is GPT-5-mini, this choice ensures that the gold labels are
not produced by the same model whose outputs are being distilled, and
in particular that the train-time cycles and conflicts cannot be
trivially memorized into the evaluation. To verify that our
conclusions are not specific to the choice of gold annotator, we also
construct a parallel gold version on the same evaluation pool using
GPT-5-mini and use it for a teacher-source robustness check
in \S\ref{sec:exp:ablation}.

